Early Time Light Curves of Type Ia Supernovae Observed with TESS

We present early time light curves of Type Ia supernovae observed in the first six sectors of TESS data. Ten of these supernovae were discovered by ASAS-SN, seven by ATLAS, six by ZTF, and one by \textit{Gaia}. For nine SNe with sufficient dynamic range ($>$3.0 mag from detection to peak), we fit power law models and search for signatures of companion stars. We find a diversity of early time light curve shapes, although most of our sources are consistent with fireball models where the flux increases $\propto t^2$. Three SN display a flatter rise with flux $\propto t$. We do not find any evidence for additional structure such as multiple power law components in the early rising light curves. For assumptions about the SN properties and the observer viewing angle, and further assuming that companion stars would be in Roche-lobe overflow, we place limits on the radii of companions for six SNe with complete coverage of the early time light curves. The upper limits are $\lesssim$\,32 R$_\odot$ for these six supernovae, $\lesssim$\,20 R$_\odot$ for five of these six, and $\lesssim$\,4 R$_\odot$ for two of these six. The small sample size does not constrain occurrence rates of single degenerate Type Ia SN progenitors, but we expect that TESS observed enough SNe in its primary mission (26 sectors) to inform this measurement. We also show that TESS is capable of detecting emission from a 1 \rsun\ companion for a Type Ia SN within 50 Mpc, and may do so after about six years.

==> table_companion_params.tex <==
\begin{deluxetable}{lrr} \tablewidth{0pt}\tablecaption{Upper limits on Companion Parameters\label{tab:companion_params}}\tablehead{\colhead{Name}&\colhead{Separation}&\colhead{Radius}\\  &\colhead{(cm)}&\colhead{(R$_{\odot}$)}  }\startdata
ATLAS-18tne & 5.1$\times 10^{12}$ & 25.1\\
ASASSN--18tb & 3.5$\times 10^{11}$ & 1.7\\
ASASSN--18ty & 2.9$\times 10^{12}$ & 14.2\\
Gaia-18czg & 6.7$\times 10^{11}$ & 3.3\\
ASASSN--18yc & 7.7$\times 10^{11}$ & 3.8\\
ZTF-18adaifep & 1.9$\times 10^{11}$ & 1.0\\
\enddata\tablecomments{Limits are derived from a fiducial model with a viewing angle of $45^{\circ}$, an ejecta mass of 1.4 M$_\odot$, a velocity of 10$^4$ km s$^{-1}$, and an opacity of 0.2 cm$^2$ g$^{-1}$.  See \S\ref{sec:models} and \citet{Kasen2010} for details.}\end{deluxetable}

